Graph Compression with Side Information at the Decoder

In this paper, we study the problem of graph compression with side information at the decoder. The focus is on the situation when an unlabelled graph (which is also referred to as a structure) is to be compressed or is available as side information. For correlated Erd\H{o}s-R\'enyi weighted random graphs, we give a precise characterization of the smallest rate at which a labelled graph or its structure can be compressed with aid of a correlated labelled graph or its structure at the decoder. We approach this problem by using the entropy-spectrum framework and establish some convergence results for conditional distributions involving structures, which play a key role in the construction of an optimal encoding and decoding scheme. Our proof essentially uses the fact that, in the considered correlated Erd\H{o}s-R\'enyi model, the structure retains most of the information about the labelled graph. Furthermore, we consider the case of unweighted graphs and present how the optimal decoding can be done using the notion of graph alignment.

==> Binary.tex <==
\section{Appendix}
\subsection{Proof of Lemma~\ref{lem:asymp:qap}} \label{proof:asymp:qap}
We will argue that 
\begin{align}
    \frac{\max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}}{\binom{n}{2}} \rightarrow p_{11}
\end{align}
in probability,  if $\frac{p_{11}p_{00}}{p_{10}p_{01}} > 1$, and the proof in the case of $\frac{p_{11}p_{00}}{p_{10}p_{01}} < 1$ follows analogously . Fix a $\delta >0$,
\begin{align}
    &\mathbb{P}\left(\left\lvert\frac{\max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}}{\binom{n}{2}} - p_{11}\right\rvert>\delta\right)\nonumber \\ & \mkern 20mu  = \mathbb{P}\left(\max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)} <  \binom{n}{2}(p_{11} - \delta)\right)+ \mathbb{P}\left( \max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}> \binom{n}{2}(p_{11} + \delta) \right) 
    \\ & \mkern 20mu  \leq \mathbb{P}\left(\sum_{i<j}\ea_{i,j}\eb_{i,j} <  \binom{n}{2}(p_{11} - \delta)\right)+ \mathbb{P}\left( \max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}> \binom{n}{2}(p_{11} + \delta) \right). \label{eq:firstterm}
\end{align}
As we know that 
\begin{align}
    \frac{\sum_{i<j}\ea_{i,j}\eb_{i,j}}{\binom{n}{2}} \to \mathbb{E}[\ea\eb]=p_{11}
\end{align}
in probability by the weak law of large numbers, the first term in \eqref{eq:firstterm} goes to zero, i.e.,  $$\mathbb{P}\left(\sum \limits_{i<j}\ea_{i,j}\eb_{i,j} <  \binom{n}{2}(p_{11} - \delta)\right) \to 0.$$
In order to deal with the second term in \eqref{eq:firstterm}, we use a concentration inequality related to a function satisfying the bounded difference property.
\begin{theorem}[Theorem~6.2, \cite{boucheron_book}]\label{thm:bdp}
    Let $\mathbf{X}=(X_1, \ldots, X_m)$ be a collection of independent random variables, and let $f: \mathcal{X}^n \to \mathbb{R}$ be a function satisfying the bounded difference property, i.e.,
    $$\sup_{\substack{x_1,\ldots,x_i, \ldots, x_m \in \mathcal{X}\\ x'_i \in \mathcal{X}}}|f(x_1,\ldots,x_i, \ldots, x_m) - f(x_1,\ldots,x'_i, \ldots, x_m)| \leq c_i$$
    for some constants $c_i$, $1 \leq i \leq m$. Then it holds that for $t>0$
    \begin{align}
        \mathbb{P}\left(f(\mathbf{X})-\mathbb{E}[f(\mathbf{X})]> t\right) \leq e^{-\frac{2t^2}{\sum_{i=1}^mc_i^2}}.
    \end{align}    
\end{theorem}

For a given permutation $\pi$, we will apply the above theorem to the function $\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}$. In  the theorem, we set $m=\binom{n}{2}$ with  $\mathbf{X}$ being the independent collection of pairs $\{(\ea_{i,j}, \eb_{i,j})\}_{i<j}$ in some order. Now, we need to compute the expectation of $f(\mathbf{X})=\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}$ and show that $f$ satisfies the bounded difference property. 

 

Suppose that a (vertex) permutation $\pi$ has $k$ fixed points\footnote{We say that $i \in [n]$ is a \emph{fixed point} of $\pi$ if $\pi(i)=i$, and call an unordered pair $\{i,j\}$ a \emph{transposition} of $\pi$ if $\pi(i)=j$ and $\pi(j)=i$.} and $t$ transpositions. Then, the number of unordered pair $\{i, j\}$ for which $\{\pi(i), \pi(j)\}=\{i, j\}$ is $l\triangleq\binom{k}{2}+ t$, which is bounded above by $\binom{n}{2}$. Here $\binom{k}{2}$ denotes the numbers of edges whose incident vertices are both fixed points of $\pi$, and  $t$ is the number of edges whose incident vertex pairs are transpositions. The rest of the edges have an incident vertex with a relabelling other than $\{i, j\}$. In the former case $\eb_{\pi(i),\pi(j)}= \eb_{i,j}$, which is correlated with $\ea_{i,j}$, and  hence $\mathbb{E}[\ea_{i,j}\eb_{\pi(i),\pi(j)}]= p_{11}$. In the latter case, $\eb_{\pi(i),\pi(j)} \neq \eb_{i,j}$, hence it is independent of  $\ea_{i,j}$, implying that $\mathbb{E}[\ea_{i,j}\eb_{\pi(i),\pi(j)}]= \mathbb{E}[\ea_{i,j}]\mathbb{E}[\eb_{\pi(i),\pi(j)}]=(p_{10}+p_{11})(p_{01}+p_{11})$. Thus,
\begin{align}
    \mathbb{E}[f(\mathbf{X})]= \mathbb{E}\left[\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}\right]= \sum_{i<j} \mathbb{E}\left[\ea_{i,j}\eb_{\pi(i),\pi(j)}\right]
& = l p_{11}+\left[\binom{n}{2}-l\right](p_{10}+p_{11})(p_{01}+p_{11}).
\end{align}
Next we will argue that $f(\mathbf{x})=\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}$ satisfies the bounded difference property with $c_{i, j}=2$ for all $i<j$. 
Fix a pair $(i_0, j_0)$.  In the sum $\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}$, the terms corresponding to $(\eea_{i_0,j_0}, \eeb_{i_0,j_0})$ are $\eea_{i_0,j_0}\eeb_{\pi(i_0),\pi(j_0)}$ and $\eea_{\pi^{-1}(i_0),\pi^{-1}(j_0)}\eeb_{i_0,j_0}$ if $\{\pi(i_0), \pi(j_0)\}\neq  \{i_0, j_0\}$; and in the other case, we only have a single term $\eea_{i_0,j_0}\eeb_{i_0,j_0}$ . Any change in the value of $(\eea_{i_0,j_0}, \eeb_{i_0,j_0})$ will only affect these terms. So, the maximum  difference in the value of $\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}$ by changing $(\eea_{i_0,j_0}, \eeb_{i_0,j_0})\in \{0,1\}^2$ to $(\teea_{i_0,j_0}, \teeb_{i_0,j_0})\in \{0,1\}^2$   is 
$$\left\lvert \eea_{i_0,j_0}\eeb_{i_0,j_0} - \teea_{i_0,j_0}\teeb_{i_0,j_0} \right\rvert \quad \text {if } \{\pi(i_0), \pi(j_0)\}= \{i_0, j_0\}$$
 and 
 $$\left\lvert (\eea_{i_0,j_0}-\teea_{i_0,j_0})\eeb_{\pi(i_0),\pi(j_0)} + \eea_{\pi^{-1}(i_0),\pi^{-1}(j_0)}(\eeb_{i_0,j_0}- \teeb_{i_0,j_0})\right\rvert \quad \text {if } \{\pi(i_0), \pi(j_0)\}= \{i_0, j_0\}.$$
In either case, these quantities are at most two. Therefore, $c_{i, j}=2$ for all $i<j$. Hence, by applying Theorem~\ref{thm:bdp} with $t= \binom{n}{2}\delta$, we obtain
\begin{align}
        \mathbb{P}\left(\sum \limits_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}-\left(l p_{11}+\left[\binom{n}{2}-l\right](p_{10}+p_{11})(p_{01}+p_{11}) \right)>\binom{n}{2}\delta\right) \leq e^{-\frac{2\binom{n}{2}^2\delta^2}{4\binom{n}{2}}} = e^{-\binom{n}{2}\frac{\delta^2}{2}}
    \end{align}  
The condition $\frac{p_{11}p_{00}}{p_{10}p_{01}}> 1$ implies the inequality  $ (p_{10}+p_{11})(p_{01}+p_{11})<p_{11}$. Therefore for any $ 0\leq l \leq \binom{n}{2}$, $l p_{11}+\left[\binom{n}{2}-l\right](p_{10}+p_{11})(p_{01}+p_{11}) \leq  \binom{n}{2} p_{11}$, which implies that 
\begin{align}
&\mathbb{P}\left(\sum \limits_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}>\binom{n}{2}p_{11}+\binom{n}{2}\delta\right)\\
& \mkern 10mu
        \leq \mathbb{P}\left(\sum \limits_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}>l p_{11}+\left[\binom{n}{2}-l\right](p_{10}+p_{11})(p_{01}+p_{11})+ \binom{n}{2}\delta \right) \leq  e^{-\binom{n}{2}\frac{\delta^2}{2}}.\label{eq:perm:bound}
    \end{align}
Observe that the above exponential bound is not dependent on the permutation $\pi$. We can finally bound the required probability involving $\max_{\pi \in \mathcal{S}_n}$ by using the union bound as follows:
\begin{align}
    \mathbb{P}\left( \max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}> \binom{n}{2}(p_{11} + \delta) \right) &\stackrel{(a)}{\leq} \sum_{\pi \in \mathcal{S}_n} \mathbb{P}\left( \sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}> \binom{n}{2}(p_{11} + \delta) \right)\\
    & \leq \sum_{\pi \in \mathcal{S}_n} e^{-\binom{n}{2}\frac{\delta^2}{2}}\\
    & = n!e^{-\binom{n}{2}\frac{\delta^2}{2}}\\
    & \leq n^ne^{-\binom{n}{2}\frac{\delta^2}{2}}\\
    & = e^{-\left[\binom{n}{2}\frac{\delta^2}{2}-n\ln n\right]},
\end{align}
where $(a)$ is due to the inequality $\eqref{eq:perm:bound}$, which holds for all $\pi \in \mathcal{S}_n$.
For a fixed $\delta>0$, the exponent $\binom{n}{2}\frac{\delta^2}{2}-n\ln n \to \infty$ as $n \to \infty$, yielding 
\begin{align}
    \mathbb{P}\left( \max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}> \binom{n}{2}(p_{11} + \delta) \right) \to 0
\end{align}
which ultimately shows the convergence in probability \eqref{eq:max:conv:prob}.



\subsection{Proof of Theorem~\ref{thm:asymp:inprob}} \label{proof:asymp:inprob}
First note that given a structure $\srel$, the number of distinct graphs having the same structure is $\frac{n!}{|\operatorname{Aut}(\srel)|}$, where $\operatorname{Aut}(\srel)$ denotes the automorphism group of a graph with the structure $\s$. Using this, we can express the conditional probability distribution as 
    \begin{align}
        P_{\ga|\s}(\gga| \srel)&= \frac{P_{\ga, \s}(\gga, \srel)}{P_{\s}(\srel)}\\
        & \stackrel{(a)}{=}  \frac{\sum \limits_{\ggb: \ggb \cong \srel} P_{\ga, \gb}(\gga, \ggb)}{\sum \limits_{\ggb: \ggb \cong \srel}P_{\gb}(\ggb)}\\
        & \stackrel{(b)}{=} \frac{\frac{1}{|\operatorname{Aut}(\srel)|}\sum \limits_{\pi \in \mathcal{S}_n, \ggb \cong \srel} P_{\ga, \gb}(\gga, \pi(\ggb))}{\frac{n!}{|\operatorname{Aut}(\srel)|}(p_{01}+p_{11})^{|\mathcal{E}(\srel)|} \cdot (p_{10}+p_{00})^{\binom{n}{2}-|\mathcal{E}(\srel)|}} \\
        & =\frac{1}{n!} \frac{\sum \limits_{\pi \in \mathcal{S}_n, \ggb \cong \srel} P_{\ga, \gb}(\gga, \pi(\ggb))}{(p_{01}+p_{11})^{|\mathcal{E}(\srel)|} \cdot (p_{10}+p_{00})^{\binom{n}{2}-|\mathcal{E}(\srel)|}}, \label{eq:ratio}
    \end{align}
where in $(a)$, we use  the notation that $\ggb \cong \srel$ to mean that the graph $\ggb$ is obtained by labelling vertices of the structure $\srel$, and in the summation in $(b)$, we fix a graph $\ggb$ such that $\ggb \cong \srel$ and apply a permutation $\pi$ to the labels to get $\pi(\ggb)$. In $(b)$, we extended the summation over all the distinct graphs having the structure $\srel$ to all permutations after fixing a graph $\ggb$ with the structure $\srel$. Since each distinct graph is obtained by applying $|\operatorname{Aut}(\srel)|$ number of permutations to $\ggb$, we get the prefactor $\frac{1}{|\operatorname{Aut}(\srel)|}$.

The summation term in \eqref{eq:ratio} can be written as 
\begin{align*}
    &\mkern -20mu \sum \limits_{\pi \in \mathcal{S}_n, \ggb \cong \srel} P_{\ga, \gb}(\gga, \pi(\ggb)) \\ 
    &= \sum \limits_{\pi \in \mathcal{S}_n, \ggb \cong \srel} \prod_{i<j} p_{00}^{(1-\eea_{i,j})(1-\eeb_{\pi(i),\pi(j)})}p_{10}^{\eea_{i,j}(1-\eeb_{\pi(i),\pi(j)})} p_{01}^{(1-\eea_{i,j})\eeb_{\pi(i),\pi(j)}}p_{11}^{\eea_{i,j}\eeb_{\pi(i),\pi(j)}}\\
    &= \sum \limits_{\pi \in \mathcal{S}_n}  p_{00}^{\binom{n}{2}}
    \left(\frac{p_{10}}{p_{00}}\right)^{\sum_{i<j}\eea_{i,j}}
    \left(\frac{p_{01}}{p_{00}}\right)^{\sum_{i<j}\eeb_{\pi(i),\pi(j)}}
    \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}}\\
    &=   p_{00}^{\binom{n}{2}}
    \left(\frac{p_{10}}{p_{00}}\right)^{|\mathcal{E}(\gga)|}
    \left(\frac{p_{01}}{p_{00}}\right)^{|\mathcal{E}(\srel)|}
    \sum \limits_{\pi \in \mathcal{S}_n} \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}},
\end{align*}
which simplifies \eqref{eq:ratio} to
\begin{align*}
        P_{\ga|\s}(\gga| \srel)&=\frac{1}{n!} \left(\frac{p_{00}}{p_{10}+p_{00}}\right)^{\binom{n}{2}}
    \left(\frac{p_{10}}{p_{00}}\right)^{|\mathcal{E}(\gga)|}
    \left(\frac{p_{01}(p_{10}+p_{00})}{p_{00}(p_{01}+p_{11})}\right)^{|\mathcal{E}(\srel)|}
    \sum \limits_{\pi \in \mathcal{S}_n} \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}}.
\end{align*}
Thus
\begin{align*}
       \frac{1}{\binom{n}{2}} \log \frac{1}{P_{\ga|\s}(\gga| \srel)}&=-\frac{\log n!}{\binom{n}{2}} - \log \left(\frac{p_{00}}{p_{10}+p_{00}}\right) - \frac{|\mathcal{E}(\gga)|}{\binom{n}{2}} \log \left(\frac{p_{10}}{p_{00}}\right)\\ &\mkern 30mu - \frac{|\mathcal{E}(\srel)|}{\binom{n}{2}}
    \log\left(\frac{p_{01}(p_{10}+p_{00})}{p_{00}(p_{01}+p_{11})}\right)  - \frac{1}{\binom{n}{2}}\log
    \left[\sum \limits_{\pi \in \mathcal{S}_n} \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\eea_{i,j}\eeb_{\pi(i),\pi(j)}}\right].
\end{align*}

By the weak law of large numbers, we know that 
\begin{align}
     \frac{|\mathcal{E}(\ga)|}{\binom{n}{2}}  \to  \mathbb{E}[\ea]=p_{10}+p_{11}  \qquad \text{and} \quad \frac{|\mathcal{E}(\s)|}{\binom{n}{2}}  \to \mathbb{E}[\eb]=  p_{01}+p_{11}  
\end{align}
in probability. 
If we are able to show that
\begin{align}\label{eq:conv:prob:log max}
    \frac{1}{\binom{n}{2}}\log
    \left[\sum \limits_{\pi \in \mathcal{S}_n} \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}}\right] \to \mathbb{E}[\ea\eb]\log\left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right) =p_{11}\log\left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right),
\end{align}
then by the linearity of convergence in probability, we will have 
\begin{align*}
       \frac{1}{\binom{n}{2}} \log \frac{1}{P_{\ga|\s}(\ga| \s)} &\to   -\log \left(\frac{p_{00}}{p_{10}+p_{00}}\right) - (p_{10}+p_{11}) \log \left(\frac{p_{10}}{p_{00}}\right) - (p_{01}+p_{11})
    \log\left(\frac{p_{01}(p_{10}+p_{00})}{p_{00}(p_{01}+p_{11})}\right)\\ & \mkern 300mu  - p_{11}\log\left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)\\
    & = -p_{00} \log \left(\frac{p_{00}}{p_{10}+p_{00}}\right) -p_{10} \log \left(\frac{p_{01}}{p_{10}+p_{00}}\right)
    -p_{11} \log \left(\frac{p_{11}}{p_{01}+p_{11}}\right) \\ & \mkern 300mu -p_{01} \log \left(\frac{p_{01}}{p_{01}+p_{11}}\right)\\
    & = H(\ea | \eb )
\end{align*}
proving the lemma. 

Now it only remains to argue \eqref{eq:conv:prob:log max}. When  $\frac{p_{11}p_{00}}{p_{10}p_{01}} > 1$,  
\begin{align}
    \left(\max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}\right)\log
    \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right) &\leq \log
    \left[\sum \limits_{\pi \in \mathcal{S}_n} \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right)^{\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}}\right]  \\ &\leq \log n! + \left(\max_{\pi \in \mathcal{S}_n}\sum_{i<j}\ea_{i,j}\eb_{\pi(i),\pi(j)}\right)\log
    \left(\frac{p_{11}p_{00}}{p_{10}p_{01}}\right).
\end{align}
If $\frac{p_{11}p_{00}}{p_{10}p_{01}} < 1$, then we will have $\min_{\pi \in \mathcal{S}_n}$ instead of $\max_{\pi \in \mathcal{S}_n}$ in the above relation. As  $\frac{\log n!}{\binom{n}{2}} \rightarrow 0$, we can apply  Lemma~\ref{lem:asymp:qap} to yield \eqref{eq:conv:prob:log max}. Note that the convergence in \eqref{eq:conv:prob:log max} is with respect to the probability distribution $P_{\ga, \s}$, and $\eb_{i,j}$'s correspond to some graph having the structure $\s$. Though we made an arbitrary choice in fixing this graph, we can show that the convergence in \eqref{eq:conv:prob:log max} is implied by the convergence in \eqref{lem:asymp:qap}, which is with respect to $P_{\ga, \gb}$.





==> Figures/sys_model_1.tex <==
\tikzstyle{block}=[rectangle, draw, thick, minimum width=2em, minimum height=2em]

\begin{tikzpicture}[node distance=4cm,auto,>=latex']
    
    \node (dummy) {};
    \node [block, align=center] (enc) [left of=dummy, node distance=2.5cm] {Encoder\\$\phi_n$};
     \node [block, align=center] (dec) [right of=dummy, node distance=4.5cm] {Decoder\\$\psi_n$};
     \node [block, align=center] (gen) [above of=dummy, node distance=3cm] {CER Model \\ $(\ga,\gb)$};
     \node (u) [left of=enc, node distance=2.5cm] {$U$};
     \node (hatu) [right of=dec, node distance=2.5cm] {$\hat{U}$};
     \node [block, align=center] (perm) [above of=dec, node distance=3cm] {Vertex-Label\\ Anonymization};
     \node [block, align=center] (perm1) [above of=u, node distance=3cm] {Vertex-Label\\ Anonymization};
     \node (m) [above of=dummy, node distance=0.5cm] {$M_n \in \big[2^{{\binom{n}{2}R}}\big]$};
     % \node (dummy2) [above of=g1, node distance=3cm] {};
     
     \draw[->, thick] (u.east) --  (enc.west);
     \draw[->, thick] (enc.east) --  (dec.west);
     \draw[->, thick] (dec.east) --  (hatu.west);
     \draw[->, thick] (perm.south) -- node[right]{$\stb$}  (dec.north) ;
     \draw[->, thick] (gen.east) -- node[above]{$\gb$} (perm.west)  ;
     \draw[->, thick] (gen.west) -- node[above]{$\ga$} (perm1.east)  ;
     \draw[->, thick] (perm1.south) --  (u.north);
     % \draw[dashed] (gen.west) --  (dummy2);
     % \draw[->, dashed] (dummy2) --  (g1.north);
     %\draw[->, dashed] (gen.west) -|  (u.north);
  

\end{tikzpicture}
